Size Should Not Matter: Evaluating Network Visualizations with Stress

The normalized stress metric is widely used to assess graph drawing quality, measuring how closely distances between vertices in a layout match their graph-theoretic distances. This metric is a standard for both evaluation and optimization in many popular graph layout algorithms. However, normalized stress is highly sensitive to the scale (size) of the drawing, leading to potentially misleading comparisons between layouts produced by different algorithms. Uniformly scaling a layout can significantly alter stress values without changing the underlying structure, even to the extent that a clearly superior layout can appear to have a higher stress score than a random layout. Although this issue is recognized within the network visualization community, it is rarely addressed with sufficient detail in publications, resulting in critical calculation errors in recent studies. In this paper, we systematically examine various stress metrics used in the literature and demonstrate that commonly used metrics are affected by layout scale, undermining their reliability for comparison. We identify scale-invariant alternatives and propose scale-normalized stress for fair stress-based evaluation.

==> tables/494-bus-comparison.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{caddf0} 8 \\
sfdp & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{e5eff9} 11 \\
GD2 (ST) & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
GD2 (NP) & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{f7fbff} 13 \\
GD2 (ST+IL) & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{bed8ec} 7 \\
GD2 (ST+NP) & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{dce9f6} 10 \\
GD2 (ST+CR) & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{a0cbe2} 5 \\
GD2 (ST+CAM) & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
GD2 (ST+AR) & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 \\
GD2 (ST+VR) & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
GD2 (ST+GB) & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{d3e3f3} 9 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{eef5fc} 12 \\
\hline
\end{tabular}
\caption{Comparison of rankings for \texttt{494-bus} graph from replicate and scale-normalized stress data.}
\label{tab:494-bus-compare}
\end{table}


==> tables/494-bus-short.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{afd1e7} 1 & \cellcolor[HTML]{caddf0} 3 \\
sfdp & \cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{e5eff9} 6 \\
GD2 (ST+IL) & \cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{bed8ec} 2 \\
GD2 (ST+NP) & \cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{dce9f6} 5 \\
GD2 (ST+CR) & \cellcolor[HTML]{bed8ec} 2 & \cellcolor[HTML]{a0cbe2} 1 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 3 & \cellcolor[HTML]{d3e3f3} 4 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{eef5fc} 7 \\
\hline
\end{tabular}
\caption{Normalized rankings for selected methods from replicate and SNS data.}
\label{{tab:filtered-normalized}}
\end{table}


==> tables/combined.tex <==
\begin{figure}[H]
\centering
\begin{minipage}{0.17\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|}
\hline
\textbf{Name} \\\hline
Neato \\
Sfdp \\
GD$^2$ (ST+IL) \\
GD$^2$ (ST+NP) \\
GD$^2$ (ST+CR) \\
GD$^2$ (ST+IL+ANR) \\
GD$^2$ (IL+NP+VR) \\
\hline
\end{tabular}
}
\subcaption*{Methods}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{afd1e7} 1 & \cellcolor[HTML]{caddf0} 3 \\
\cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{e5eff9} 6 \\
\cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{bed8ec} 2 \\
\cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{dce9f6} 5 \\
\cellcolor[HTML]{bed8ec} 2 & \cellcolor[HTML]{a0cbe2} 1 \\
\cellcolor[HTML]{caddf0} 3 & \cellcolor[HTML]{d3e3f3} 4 \\
\cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{eef5fc} 7 \\
\hline
\end{tabular}
}
\subcaption*{494-bus}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{a0cbe2} 2 & \cellcolor[HTML]{afd1e7} 3 \\
\cellcolor[HTML]{7ab6d9} 1 & \cellcolor[HTML]{7ab6d9} 1 \\
\cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{d3e3f3} 5 \\
\cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{eef5fc} 6 \\
\cellcolor[HTML]{f7fbff} 7 & \cellcolor[HTML]{f7fbff} 7 \\
\cellcolor[HTML]{caddf0} 4 & \cellcolor[HTML]{a0cbe2} 2 \\
\cellcolor[HTML]{afd1e7} 3 & \cellcolor[HTML]{bed8ec} 4 \\
\hline
\end{tabular}
}
\subcaption*{Dodecahed.}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
\cellcolor[HTML]{bed8ec} 3 & \cellcolor[HTML]{d3e3f3} 4 \\
\cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{bed8ec} 3 \\
\cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{dce9f6} 5 \\
\cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{e5eff9} 6 \\
\cellcolor[HTML]{afd1e7} 2 & \cellcolor[HTML]{afd1e7} 2 \\
\cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{f7fbff} 7 \\
\hline
\end{tabular}
}
\subcaption*{Dwt-1005}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{8dc1dd} 2 & \cellcolor[HTML]{8dc1dd} 2 \\
\cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
\cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{d3e3f3} 5 \\
\cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{eef5fc} 7 \\
\cellcolor[HTML]{bed8ec} 3 & \cellcolor[HTML]{caddf0} 4 \\
\cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{bed8ec} 3 \\
\cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{e5eff9} 6 \\
\hline
\end{tabular}
}
\subcaption*{Dwt-307}
\end{minipage}
\\[1ex]
% Second row of tables
\begin{minipage}{0.17\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|}
\hline
\textbf{Name} \\\hline
Neato \\
Sfdp \\
GD$^2$ (ST+IL) \\
GD$^2$ (ST+NP) \\
GD$^2$ (ST+CR) \\
GD$^2$ (ST+IL+ANR) \\
GD$^2$ (IL+NP+VR) \\
\hline
\end{tabular}
}
\subcaption*{Methods}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{69add5} 1 & \cellcolor[HTML]{69add5} 1 \\
\cellcolor[HTML]{caddf0} 3 & \cellcolor[HTML]{dce9f6} 5 \\
\cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{caddf0} 3 \\
\cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{eef5fc} 7 \\
\cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{e5eff9} 6 \\
\cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{d3e3f3} 4 \\
\cellcolor[HTML]{bed8ec} 2 & \cellcolor[HTML]{afd1e7} 2 \\
\hline
\end{tabular}
}
\subcaption*{Grid-12-24}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{8dc1dd} 1 & \cellcolor[HTML]{8dc1dd} 1 \\
\cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{e5eff9} 6 \\
\cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{dce9f6} 5 \\
\cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{d3e3f3} 4 \\
\cellcolor[HTML]{a0cbe2} 2 & \cellcolor[HTML]{a0cbe2} 2 \\
\cellcolor[HTML]{caddf0} 3 & \cellcolor[HTML]{caddf0} 3 \\
\cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{eef5fc} 7 \\
\hline
\end{tabular}
}
\subcaption*{Grid1}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{8dc1dd} 1 & \cellcolor[HTML]{8dc1dd} 1 \\
\cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{e5eff9} 6 \\
\cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{dce9f6} 5 \\
\cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{d3e3f3} 4 \\
\cellcolor[HTML]{a0cbe2} 2 & \cellcolor[HTML]{a0cbe2} 2 \\
\cellcolor[HTML]{caddf0} 3 & \cellcolor[HTML]{caddf0} 3 \\
\cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{eef5fc} 7 \\
\hline
\end{tabular}
}
\subcaption*{Spx-teaser}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{8dc1dd} 1 & \cellcolor[HTML]{8dc1dd} 1 \\
\cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{e5eff9} 6 \\
\cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{dce9f6} 5 \\
\cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{d3e3f3} 4 \\
\cellcolor[HTML]{a0cbe2} 2 & \cellcolor[HTML]{a0cbe2} 2 \\
\cellcolor[HTML]{caddf0} 3 & \cellcolor[HTML]{caddf0} 3 \\
\cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{eef5fc} 7 \\
\hline
\end{tabular}
}
\subcaption*{Tree-2-6}
\end{minipage}
\caption{The replicated ranking of results from~\cite{ahmed2022multicriteria} and the ranking of scale-normalized stress are compared. This comparison demonstrates that the results can change when scale is taken into account.}
\label{tab:filtered-normalized}
\end{figure}


==> tables/combined_correct.tex <==
\begin{figure}[H]
\centering
\begin{minipage}{0.17\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|}
\hline
\textbf{Name} \\\hline
Neato \\
Sfdp \\
GD$^2$ (ST+IL) \\
GD$^2$ (ST+NP) \\
GD$^2$ (ST+CR) \\
GD$^2$ (ST+IL+ANR) \\
GD$^2$ (IL+NP+VR) \\
\hline
\end{tabular}
}
\subcaption*{Methods}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{7ab6d9} 3 \\
\cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 \\
\cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{69add5} 2 \\
\cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{a0cbe2} 5 \\
\cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{5aa2cf} 1 \\
\cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{8dc1dd} 4 \\
\cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{bed8ec} 7 \\
\hline
\end{tabular}
}
\subcaption*{494-bus}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{7ab6d9} 3 \\
\cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
\cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{a0cbe2} 5 \\
\cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{afd1e7} 6 \\
\cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{bed8ec} 7 \\
\cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{69add5} 2 \\
\cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{8dc1dd} 4 \\
\hline
\end{tabular}
}
\subcaption*{Dodecahed.}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
\cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{8dc1dd} 4 \\
\cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{7ab6d9} 3 \\
\cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{a0cbe2} 5 \\
\cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 \\
\cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
\cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{bed8ec} 7 \\
\hline
\end{tabular}
}
\subcaption*{Dwt-1005}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
\cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
\cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{a0cbe2} 5 \\
\cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{bed8ec} 7 \\
\cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{8dc1dd} 4 \\
\cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{7ab6d9} 3 \\
\cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 \\
\hline
\end{tabular}
}
\subcaption*{Dwt-307}
\end{minipage}
\\[1ex]
% Second row of tables
\begin{minipage}{0.17\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|}
\hline
\textbf{Name} \\\hline
Neato \\
Sfdp \\
GD$^2$ (ST+IL) \\
GD$^2$ (ST+NP) \\
GD$^2$ (ST+CR) \\
GD$^2$ (ST+IL+ANR) \\
GD$^2$ (IL+NP+VR) \\
\hline
\end{tabular}
}
\subcaption*{Methods}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
\cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{a0cbe2} 5 \\
\cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{7ab6d9} 3 \\
\cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{bed8ec} 7 \\
\cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{afd1e7} 6 \\
\cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{8dc1dd} 4 \\
\cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
\hline
\end{tabular}
}
\subcaption*{Grid-12-24}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
\cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 \\
\cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{a0cbe2} 5 \\
\cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
\cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
\cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
\cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{bed8ec} 7 \\
\hline
\end{tabular}
}
\subcaption*{Grid1}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
\cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 \\
\cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{a0cbe2} 5 \\
\cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
\cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
\cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
\cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{bed8ec} 7 \\
\hline
\end{tabular}
}
\subcaption*{Spx-teaser}
\end{minipage}%
\begin{minipage}{0.12\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Rep.} & \textbf{SNS} \\\hline
\cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
\cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 \\
\cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{a0cbe2} 5 \\
\cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
\cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
\cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
\cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{bed8ec} 7 \\
\hline
\end{tabular}
}
\subcaption*{Tree-2-6}
\end{minipage}
\caption{The replicated ranking of results from~\cite{ahmed2022multicriteria} and the ranking of scale-normalized stress are compared. This comparison demonstrates that the results can change when scale is taken into account.}
\label{tab:filtered-normalized}
\end{figure}


==> tables/diff-494-bus-comparison.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{caddf0} 8 \\
sfdp & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{e5eff9} 11 \\
GD2 (ST+IL) & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{bed8ec} 7 \\
GD2 (ST+NP) & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{dce9f6} 10 \\
GD2 (ST+CR) & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{a0cbe2} 5 \\
GD2 (ST+AR) & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{d3e3f3} 9 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{eef5fc} 12 \\
\hline
\end{tabular}
\caption{Methods with differing rankings for \texttt{494-bus} graph from replicate and scale-normalized stress data.}
\label{tab:494-bus-diff-ranks}
\end{table}


==> tables/dodecahedron-comparison.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 \\
sfdp & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
GD2 (ST) & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
GD2 (NP) & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{e5eff9} 11 \\
GD2 (ST+IL) & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{d3e3f3} 9 \\
GD2 (ST+NP) & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{eef5fc} 12 \\
GD2 (ST+CR) & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{f7fbff} 13 \\
GD2 (ST+CAM) & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{dce9f6} 10 \\
GD2 (ST+AR) & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
GD2 (ST+VR) & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{caddf0} 8 \\
GD2 (ST+GB) & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{a0cbe2} 5 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{bed8ec} 7 \\
\hline
\end{tabular}
\caption{Comparison of rankings for \texttt{dodecahedron} graph from replicate and scale-normalized stress data.}
\label{tab:dodecahedron-compare}
\end{table}


==> tables/dodecahedron-short.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{a0cbe2} 2 & \cellcolor[HTML]{afd1e7} 3 \\
sfdp & \cellcolor[HTML]{7ab6d9} 1 & \cellcolor[HTML]{7ab6d9} 1 \\
GD2 (ST+IL) & \cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{d3e3f3} 5 \\
GD2 (ST+NP) & \cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{eef5fc} 6 \\
GD2 (ST+CR) & \cellcolor[HTML]{f7fbff} 7 & \cellcolor[HTML]{f7fbff} 7 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 4 & \cellcolor[HTML]{a0cbe2} 2 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{afd1e7} 3 & \cellcolor[HTML]{bed8ec} 4 \\
\hline
\end{tabular}
\caption{Normalized rankings for selected methods from replicate and SNS data.}
\label{{tab:filtered-normalized}}
\end{table}


==> tables/dwt-1005-comparison.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
sfdp & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{d3e3f3} 9 \\
GD2 (ST) & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
GD2 (NP) & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{eef5fc} 12 \\
GD2 (ST+IL) & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{bed8ec} 7 \\
GD2 (ST+NP) & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{dce9f6} 10 \\
GD2 (ST+CR) & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{e5eff9} 11 \\
GD2 (ST+CAM) & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{caddf0} 8 \\
GD2 (ST+AR) & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{a0cbe2} 5 \\
GD2 (ST+VR) & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
GD2 (ST+GB) & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{afd1e7} 6 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{f7fbff} 13 \\
\hline
\end{tabular}
\caption{Comparison of rankings for \texttt{dwt-1005} graph from replicate and scale-normalized stress data.}
\label{tab:dwt-1005-compare}
\end{table}


==> tables/dwt-1005-short.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
sfdp & \cellcolor[HTML]{bed8ec} 3 & \cellcolor[HTML]{d3e3f3} 4 \\
GD2 (ST+IL) & \cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{bed8ec} 3 \\
GD2 (ST+NP) & \cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{dce9f6} 5 \\
GD2 (ST+CR) & \cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{e5eff9} 6 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{afd1e7} 2 & \cellcolor[HTML]{afd1e7} 2 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{f7fbff} 7 \\
\hline
\end{tabular}
\caption{Normalized rankings for selected methods from replicate and SNS data.}
\label{{tab:filtered-normalized}}
\end{table}


==> tables/dwt-307-comparison.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
sfdp & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
GD2 (ST) & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
GD2 (NP) & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{f7fbff} 13 \\
GD2 (ST+IL) & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{d3e3f3} 9 \\
GD2 (ST+NP) & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{eef5fc} 12 \\
GD2 (ST+CR) & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{caddf0} 8 \\
GD2 (ST+CAM) & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{dce9f6} 10 \\
GD2 (ST+AR) & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{a0cbe2} 5 \\
GD2 (ST+VR) & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{afd1e7} 6 \\
GD2 (ST+GB) & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{bed8ec} 7 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{e5eff9} 11 \\
\hline
\end{tabular}
\caption{Comparison of rankings for \texttt{dwt-307} graph from replicate and scale-normalized stress data.}
\label{tab:dwt-307-compare}
\end{table}


==> tables/dwt-307-short.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{8dc1dd} 2 & \cellcolor[HTML]{8dc1dd} 2 \\
sfdp & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
GD2 (ST+IL) & \cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{d3e3f3} 5 \\
GD2 (ST+NP) & \cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{eef5fc} 7 \\
GD2 (ST+CR) & \cellcolor[HTML]{bed8ec} 3 & \cellcolor[HTML]{caddf0} 4 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{bed8ec} 3 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{e5eff9} 6 \\
\hline
\end{tabular}
\caption{Normalized rankings for selected methods from replicate and SNS data.}
\label{{tab:filtered-normalized}}
\end{table}


==> tables/grid-12-24-comparison.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
sfdp & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{dce9f6} 10 \\
GD2 (ST) & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
GD2 (NP) & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{f7fbff} 13 \\
GD2 (ST+IL) & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{bed8ec} 7 \\
GD2 (ST+NP) & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{afd1e7} 6 \\
GD2 (ST+CR) & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
GD2 (ST+CAM) & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{d3e3f3} 9 \\
GD2 (ST+AR) & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{e5eff9} 11 \\
GD2 (ST+VR) & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{a0cbe2} 5 \\
GD2 (ST+GB) & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{caddf0} 8 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{eef5fc} 12 \\
\hline
\end{tabular}
\caption{Comparison of rankings for \texttt{grid-12-24} graph from replicate and scale-normalized stress data.}
\label{tab:grid-12-24-compare}
\end{table}


==> tables/grid-12-24-short.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
sfdp & \cellcolor[HTML]{d3e3f3} 5 & \cellcolor[HTML]{dce9f6} 6 \\
GD2 (ST+IL) & \cellcolor[HTML]{dce9f6} 6 & \cellcolor[HTML]{bed8ec} 4 \\
GD2 (ST+NP) & \cellcolor[HTML]{afd1e7} 3 & \cellcolor[HTML]{afd1e7} 3 \\
GD2 (ST+CR) & \cellcolor[HTML]{8dc1dd} 2 & \cellcolor[HTML]{8dc1dd} 2 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 4 & \cellcolor[HTML]{caddf0} 5 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{eef5fc} 7 \\
\hline
\end{tabular}
\caption{Normalized rankings for selected methods from replicate and SNS data.}
\label{{tab:filtered-normalized}}
\end{table}


==> tables/grid1-comparison.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
sfdp & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{dce9f6} 10 \\
GD2 (ST) & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
GD2 (NP) & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{f7fbff} 13 \\
GD2 (ST+IL) & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{caddf0} 8 \\
GD2 (ST+NP) & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{eef5fc} 12 \\
GD2 (ST+CR) & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{e5eff9} 11 \\
GD2 (ST+CAM) & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{a0cbe2} 5 \\
GD2 (ST+AR) & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{bed8ec} 7 \\
GD2 (ST+VR) & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
GD2 (ST+GB) & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{d3e3f3} 9 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{afd1e7} 6 \\
\hline
\end{tabular}
\caption{Comparison of rankings for \texttt{grid1} graph from replicate and scale-normalized stress data.}
\label{tab:grid1-compare}
\end{table}


==> tables/grid1-short.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{69add5} 1 & \cellcolor[HTML]{69add5} 1 \\
sfdp & \cellcolor[HTML]{caddf0} 3 & \cellcolor[HTML]{dce9f6} 5 \\
GD2 (ST+IL) & \cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{caddf0} 3 \\
GD2 (ST+NP) & \cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{eef5fc} 7 \\
GD2 (ST+CR) & \cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{e5eff9} 6 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{d3e3f3} 4 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{bed8ec} 2 & \cellcolor[HTML]{afd1e7} 2 \\
\hline
\end{tabular}
\caption{Normalized rankings for selected methods from replicate and SNS data.}
\label{{tab:filtered-normalized}}
\end{table}


==> tables/norm-494-bus-comparison.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{afd1e7} 2 & \cellcolor[HTML]{caddf0} 4 \\
sfdp & \cellcolor[HTML]{dce9f6} 6 & \cellcolor[HTML]{e5eff9} 7 \\
GD2 (ST+IL) & \cellcolor[HTML]{d3e3f3} 5 & \cellcolor[HTML]{bed8ec} 3 \\
GD2 (ST+NP) & \cellcolor[HTML]{eef5fc} 8 & \cellcolor[HTML]{dce9f6} 6 \\
GD2 (ST+CR) & \cellcolor[HTML]{bed8ec} 3 & \cellcolor[HTML]{a0cbe2} 1 \\
GD2 (ST+AR) & \cellcolor[HTML]{a0cbe2} 1 & \cellcolor[HTML]{afd1e7} 2 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 4 & \cellcolor[HTML]{d3e3f3} 5 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{e5eff9} 7 & \cellcolor[HTML]{eef5fc} 8 \\
\hline
\end{tabular}
\caption{Normalized (1–8) rankings for methods with differing performance on \texttt{494-bus} graph.}
\label{tab:494-bus-normalized}
\end{table}


==> tables/sgd-replicate.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{l c c c c c c c c c c c c c}
 & \rotatebox{70}{ neato} & \rotatebox{70}{ sfdp} & \rotatebox{70}{\tiny GD2 (ST)} & \rotatebox{70}{\tiny GD2 (NP)} & \rotatebox{70}{\tiny GD2 (ST+IL)} & \rotatebox{70}{\tiny GD2 (ST+NP)} & \rotatebox{70}{\tiny GD2 (ST+CR)} & \rotatebox{70}{\tiny GD2 (ST+CAM)} & \rotatebox{70}{\tiny GD2 (ST+AR)} & \rotatebox{70}{\tiny GD2 (ST+VR)} & \rotatebox{70}{\tiny GD2 (ST+GB)} & \rotatebox{70}{\tiny GD2 (ST+IL+ANR)} & \rotatebox{70}{\tiny GD2 (IL+NP+VR)}\\\hline



dodecahedron & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{afd1e7} 6\\\hline
tree-2-6 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{e5eff9} 11\\\hline
grid-12-24 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{eef5fc} 12\\\hline
spx-teaser & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{eef5fc} 12\\\hline
494-bus & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{e5eff9} 11\\\hline
grid1 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{bed8ec} 7\\\hline
dwt-307 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{dce9f6} 10\\\hline
dwt-1005 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{eef5fc} 12\\\hline
    \end{tabular}
    \vspace{0.25cm}
    \caption{Ranking of results from~\cite{ahmed2022multicriteria} as they appeared in the original paper (online version). Stress values have been converted to ranks across the rows, $1,2,3,\dots$ indicates the first, second, third, etc. smallest (normalized) stress scores.}
    \label{tab:sgd-res1}
    \vspace{-0.25cm}
\end{table*}


==> tables/sgd-sns.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{l c c c c c c c c c c c c c}

 & \rotatebox{70}{ neato} & \rotatebox{70}{ sfdp} & \rotatebox{70}{\tiny GD2 (ST)} & \rotatebox{70}{\tiny GD2 (NP)} & \rotatebox{70}{\tiny GD2 (ST+IL)} & \rotatebox{70}{\tiny GD2 (ST+NP)} & \rotatebox{70}{\tiny GD2 (ST+CR)} & \rotatebox{70}{\tiny GD2 (ST+CAM)} & \rotatebox{70}{\tiny GD2 (ST+AR)} & \rotatebox{70}{\tiny GD2 (ST+VR)} & \rotatebox{70}{\tiny GD2 (ST+GB)} & \rotatebox{70}{\tiny GD2 (ST+IL+ANR)} & \rotatebox{70}{\tiny GD2 (IL+NP+VR)}\\\hline
dodecahedron & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{bed8ec} 7\\\hline
tree-2-6 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{e5eff9} 11\\\hline
grid-12-24 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{eef5fc} 12\\\hline
spx-teaser & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{eef5fc} 12\\\hline
494-bus & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{eef5fc} 12\\\hline
grid1 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{afd1e7} 6\\\hline
dwt-307 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{e5eff9} 11\\\hline
dwt-1005 & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{f7fbff} 13\\\hline
    \end{tabular}
    \vspace{0.25cm}
    \caption{Ranking of results from~\cite{ahmed2022multicriteria} using scale-normalized stress. The drawings for each cell are left unchanged from ~\autoref{tab:sgd-res1}, the only difference is that scale-normalized stress is computed instead. While the rankings change only subtly, they demonstrate that results can change when taking scale into account.}
    \label{tab:sgd-res2}
    \vspace{-0.25cm}
\end{table*}

==> tables/spx-teaser-comparison.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
sfdp & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{e5eff9} 11 \\
GD2 (ST) & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
GD2 (NP) & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{f7fbff} 13 \\
GD2 (ST+IL) & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{dce9f6} 10 \\
GD2 (ST+NP) & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{d3e3f3} 9 \\
GD2 (ST+CR) & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{a0cbe2} 5 \\
GD2 (ST+CAM) & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{afd1e7} 6 \\
GD2 (ST+AR) & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
GD2 (ST+VR) & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{bed8ec} 7 \\
GD2 (ST+GB) & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{caddf0} 8 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{eef5fc} 12 \\
\hline
\end{tabular}
\caption{Comparison of rankings for \texttt{spx-teaser} graph from replicate and scale-normalized stress data.}
\label{tab:spx-teaser-compare}
\end{table}


==> tables/spx-teaser-short.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{8dc1dd} 1 & \cellcolor[HTML]{8dc1dd} 1 \\
sfdp & \cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{e5eff9} 6 \\
GD2 (ST+IL) & \cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{dce9f6} 5 \\
GD2 (ST+NP) & \cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{d3e3f3} 4 \\
GD2 (ST+CR) & \cellcolor[HTML]{a0cbe2} 2 & \cellcolor[HTML]{a0cbe2} 2 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 3 & \cellcolor[HTML]{caddf0} 3 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{eef5fc} 7 \\
\hline
\end{tabular}
\caption{Normalized rankings for selected methods from replicate and SNS data.}
\label{{tab:filtered-normalized}}
\end{table}


==> tables/tree-2-6-comparison.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{8dc1dd} 4 & \cellcolor[HTML]{8dc1dd} 4 \\
sfdp & \cellcolor[HTML]{eef5fc} 12 & \cellcolor[HTML]{f7fbff} 13 \\
GD2 (ST) & \cellcolor[HTML]{69add5} 2 & \cellcolor[HTML]{69add5} 2 \\
GD2 (NP) & \cellcolor[HTML]{f7fbff} 13 & \cellcolor[HTML]{eef5fc} 12 \\
GD2 (ST+IL) & \cellcolor[HTML]{d3e3f3} 9 & \cellcolor[HTML]{bed8ec} 7 \\
GD2 (ST+NP) & \cellcolor[HTML]{dce9f6} 10 & \cellcolor[HTML]{dce9f6} 10 \\
GD2 (ST+CR) & \cellcolor[HTML]{a0cbe2} 5 & \cellcolor[HTML]{a0cbe2} 5 \\
GD2 (ST+CAM) & \cellcolor[HTML]{5aa2cf} 1 & \cellcolor[HTML]{5aa2cf} 1 \\
GD2 (ST+AR) & \cellcolor[HTML]{bed8ec} 7 & \cellcolor[HTML]{caddf0} 8 \\
GD2 (ST+VR) & \cellcolor[HTML]{afd1e7} 6 & \cellcolor[HTML]{afd1e7} 6 \\
GD2 (ST+GB) & \cellcolor[HTML]{7ab6d9} 3 & \cellcolor[HTML]{7ab6d9} 3 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 8 & \cellcolor[HTML]{d3e3f3} 9 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{e5eff9} 11 & \cellcolor[HTML]{e5eff9} 11 \\
\hline
\end{tabular}
\caption{Comparison of rankings for \texttt{tree-2-6} graph from replicate and scale-normalized stress data.}
\label{tab:tree-2-6-compare}
\end{table}


==> tables/tree-2-6-short.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lcc}
Method & Replicate Rank & SNS Rank \\\hline
neato & \cellcolor[HTML]{8dc1dd} 1 & \cellcolor[HTML]{8dc1dd} 1 \\
sfdp & \cellcolor[HTML]{eef5fc} 7 & \cellcolor[HTML]{f7fbff} 7 \\
GD2 (ST+IL) & \cellcolor[HTML]{d3e3f3} 4 & \cellcolor[HTML]{bed8ec} 3 \\
GD2 (ST+NP) & \cellcolor[HTML]{dce9f6} 5 & \cellcolor[HTML]{dce9f6} 5 \\
GD2 (ST+CR) & \cellcolor[HTML]{a0cbe2} 2 & \cellcolor[HTML]{a0cbe2} 2 \\
GD2 (ST+IL+ANR) & \cellcolor[HTML]{caddf0} 3 & \cellcolor[HTML]{d3e3f3} 4 \\
GD2 (IL+NP+VR) & \cellcolor[HTML]{e5eff9} 6 & \cellcolor[HTML]{e5eff9} 6 \\
\hline
\end{tabular}
\caption{Normalized rankings for selected methods from replicate and SNS data.}
\label{{tab:filtered-normalized}}
\end{table}

